AI-Assisted NLOS Sensing for RIS-Based Indoor Localization in Smart Factories

In the era of Industry 4.0, precise indoor localization is vital for automation and efficiency in smart factories. Reconfigurable Intelligent Surfaces (RIS) are emerging as key enablers in 6G networks for joint sensing and communication. However, RIS faces significant challenges in Non-Line-of-Sight (NLOS) and multipath propagation, particularly in localization scenarios, where detecting NLOS conditions is crucial for ensuring not only reliable results and increased connectivity but also the safety of smart factory personnel. This study introduces an AI-assisted framework employing a Convolutional Neural Network (CNN) customized for accurate Line-of-Sight (LOS) and Non-Line-of-Sight (NLOS) classification to enhance RIS-based localization using measured, synthetic, mixed-measured, and mixed-synthetic experimental data, that is, original, augmented, slightly noisy, and highly noisy data, respectively. Validated through such data from three different environments, the proposed customized-CNN (cCNN) model achieves {95.0\%-99.0\%} accuracy, outperforming standard pre-trained models like Visual Geometry Group 16 (VGG-16) with an accuracy of {85.5\%-88.0\%}. By addressing RIS limitations in NLOS scenarios, this framework offers scalable and high-precision localization solutions for 6G-enabled smart factories.

==> 1_Abstract/Index.tex <==
\input{AI-Assisted_NLOS_Sensing_for_RIS-Based_Indoor_Localization_in_Smart_Factories/1_Abstract/Abstract.tex}

==> 2_Introduction/Index.tex <==
\input{AI-Assisted_NLOS_Sensing_for_RIS-Based_Indoor_Localization_in_Smart_Factories/2_Introduction/Introduction.tex}

==> 3_Method/Index.tex <==
\input{AI-Assisted_NLOS_Sensing_for_RIS-Based_Indoor_Localization_in_Smart_Factories/3_Method/Method.tex}

==> 4_Results/Index.tex <==
\input{AI-Assisted_NLOS_Sensing_for_RIS-Based_Indoor_Localization_in_Smart_Factories/4_Results/Results.tex}

==> 5_Conclusion/Index.tex <==
\input{AI-Assisted_NLOS_Sensing_for_RIS-Based_Indoor_Localization_in_Smart_Factories/5_Conclusion/Conclusion.tex}

==> bib/Mybib.tex <==
% BIBLIOTEK
\begin{thebibliography}{1}
\bibitem {1}
N. Wu, X. Wang, Z. Fei, F. Xia, J. Huang and A. Nallanathan, "RIS-Assisted Integrated Sensing and Backscatter Communications for Future IoT Networks," in IEEE Internet of Things Magazine, vol. 7, no. 4, pp. 44-50, July 2024, doi: 10.1109/IOTM.001.2300184.

\bibitem {2}
A. Kubota, S. Sampei and T. Takahashi, "A Study on Conversion of NLoS to LoS conditions using Sidelink in Smart Factory Environments," 2021 IEEE VTS 17th Asia Pacific Wireless Communications Symposium (APWCS), Osaka, Japan, 2021, pp. 1-5, doi: 10.1109/APWCS50173.2021.9548715.


\bibitem {3}
O. Rinch, A. Elzanaty and A. Alsharoa, "Enhancing Near-Field Wireless Localization With LiDAR-Assisted RIS in Multipath Environments," in IEEE Wireless Communications Letters, vol. 12, no. 12, pp. 2168-2172, Dec. 2023, doi: 10.1109/LWC.2023.3311730.


\bibitem {4}
O. Rinchi, A. Elzanaty and M. -S. Alouini, "Compressive Near-Field Localization for Multipath RIS-Aided Environments," in IEEE Communications Letters, vol. 26, no. 6, pp. 1268-1272, June 2022, doi: 10.1109/LCOMM.2022.3151036.


\bibitem {5}
R. Ghazalian, K. Keykhosravi, H. Chen, H. Wymeersch and R. Jäntti, "Bi-Static Sensing for Near-Field RIS Localization," GLOBECOM 2022 - 2022 IEEE Global Communications Conference, Rio de Janeiro, Brazil, 2022, pp. 6457-6462, doi: 10.1109/GLOBECOM48099.2022.10001209.


\bibitem {6}
O. Rinchi, A. Elzanaty and A. Alsharoa, "Single-Snapshot Localization for Near-Field RIS Model Using Atomic Norm Minimization," GLOBECOM 2022 - 2022 IEEE Global Communications Conference, Rio de Janeiro, Brazil, 2022, pp. 2432-2437, doi: 10.1109/GLOBECOM48099.2022.10000689.


\bibitem {7}
Z. Li, Z. Wan, K. Ying, Y. Mei, M. Ke and Z. Gao, "Reconfigurable Intelligent Surface Assisted Localization Over Near-Field Beam Squint Effect," 2022 International Symposium on Wireless Communication Systems (ISWCS), Hangzhou, China, 2022, pp. 1-6, doi: 10.1109/ISWCS56560.2022.9940428.

\bibitem {8}
N. González-Prelcic et al., "The Integrated Sensing and Communication Revolution for 6G: Vision, Techniques, and Applications," in Proceedings of the IEEE, vol. 112, no. 7, pp. 676-723, July 2024, doi: 10.1109/JPROC.2024.3397609.


\bibitem {9}
Z. Gong, L. Wu, Z. Zhang, J. Dang, Y. Wu and J. Wang, "Asynchronous RIS-Assisted Localization: A Comprehensive Analysis of Fundamental Limits," in IEEE Transactions on Wireless Communications, vol. 23, no. 9, pp. 10974-10989, Sept. 2024, doi: 10.1109/TWC.2024.3377367.


\bibitem {10}
Z. Li, Z. Gao and T. Li, "Sensing User's Channel and Location With Terahertz Extra-Large Reconfigurable Intelligent Surface Under Hybrid-Field Beam Squint Effect," in IEEE Journal of Selected Topics in Signal Processing, vol. 17, no. 4, pp. 893-911, July 2023, doi: 10.1109/JSTSP.2023.3278942.


\bibitem {11}
Y. Han, S. Jin, C. -K. Wen and T. Q. S. Quek, "Localization and Channel Reconstruction for Extra Large RIS-Assisted Massive MIMO Systems," in IEEE Journal of Selected Topics in Signal Processing, vol. 16, no. 5, pp. 1011-1025, Aug. 2022, doi: 10.1109/JSTSP.2022.3174654.


\bibitem {12}
M. Li, S. Zhang, Y. Ge, Z. Li, F. Gao and P. Fan, "STAR-RIS Aided Integrated Sensing and Communication Over High Mobility Scenario," in IEEE Transactions on Communications, vol. 72, no. 8, pp. 4788-4802, Aug. 2024, doi: 10.1109/TCOMM.2024.3381725.


\bibitem {13}
Y. Cheng, J. Du, J. Liu, L. Jin, X. Li and D. B. da Costa, "Nested Tensor-Based Framework for ISAC Assisted by Reconfigurable Intelligent Surface," in IEEE Transactions on Vehicular Technology, vol. 73, no. 3, pp. 4412-4417, March 2024, doi: 10.1109/TVT.2023.3324448.


\bibitem {14}
Z. Wang, Z. Liu, Y. Shen, A. Conti and M. Z. Win, "Location Awareness in Beyond 5G Networks via Reconfigurable Intelligent Surfaces," in IEEE Journal on Selected Areas in Communications, vol. 40, no. 7, pp. 2011-2025, July 2022, doi: 10.1109/JSAC.2022.3155542.


\bibitem {15}
F. Wang, X. Houv, X. Wang, X. Li, L. Chen and T. Asai, "Reconfigurable Intelligent Surface Aided Joint Communication And Positioning," 2023 IEEE 98th Vehicular Technology Conference (VTC2023-Fall), Hong Kong, Hong Kong, 2023, pp. 1-6, doi: 10.1109/VTC2023-Fall60731.2023.10333393.


\bibitem {16}
Hassouna, S., Jamshed, M.A., Ur-Rehman, M. et al. RIS-assisted near-field localization using practical phase shift model. Sci Rep 14, 4350 (2024). https://doi.org/10.1038/s41598-024-54859-3.

\bibitem {17}
P. Li et al., "Design of Low-Cost Single-Layer 2-Bit Reflective Programmable Metasurface Based on Folded Ground," in IEEE Transactions on Microwave Theory and Techniques, vol. 71, no. 8, pp. 3455-3465, Aug. 2023, doi: 10.1109/TMTT.2023.3259526.

\bibitem {18}
E. C. Strinati et al., "Distributed Intelligent Integrated Sensing and Communications: The 6G-DISAC Approach," 2024 Joint European Conference on Networks and Communications and 6G Summit (EuCNC/6G Summit), Antwerp, Belgium, 2024, pp. 392-397, doi: 10.1109/EuCNC/6GSummit60053.2024.10597016.

\bibitem {19}
A. Albanese, P. Mursia, V. Sciancalepore and X. Costa-Pérez, "PAPIR: Practical RIS-aided Localization via Statistical User Information," 2021 IEEE 22nd International Workshop on Signal Processing Advances in Wireless Communications (SPAWC), Lucca, Italy, 2021, pp. 531-535, doi: 10.1109/SPAWC51858.2021.9593204.

\bibitem {20}
G. Encinas-Lago, F. Devoti, M. Rossanese, V. Sciancalepore, M. D. Renzo, X. Costa-Pérez, "COLoRIS: Localization-agnostic Smart Surfaces Enabling Opportunistic ISAC in 6G Networks", Networking and Internet Architecture, doi:https://doi.org/10.48550/arXiv.2406.07377.

\end{thebibliography}
